AutoInit: Automatic Initialization via Jacobian Tuning

Good initialization is essential for training Deep Neural Networks (DNNs). Oftentimes such initialization is found through a trial and error approach, which has to be applied anew every time an architecture is substantially modified, or inherited from smaller size networks leading to sub-optimal initialization. In this work we introduce a new and cheap algorithm, that allows one to find a good initialization automatically, for general feed-forward DNNs. The algorithm utilizes the Jacobian between adjacent network blocks to tune the network hyperparameters to criticality. We solve the dynamics of the algorithm for fully connected networks with ReLU and derive conditions for its convergence. We then extend the discussion to more general architectures with BatchNorm and residual connections. Finally, we apply our method to ResMLP and VGG architectures, where the automatic one-shot initialization found by our method shows good performance on vision tasks.

==> NeurIPS Automatic Initialization/SM.tex <==
\appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Details}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Cref{fig:relu_jac}: The the second panel is made of 1200 points, each point takes around $1.5$ minutes running on a single single NVIDIA RTX 3090 GPU.

\Cref{fig:bn_relu}: We scanned over $400$ points for each phase diagram, which overall takes around $5$ hours on a single NVIDIA RTX 3090 GPU.

\Cref{fig:resmlp}: We use \cref{alg:j_train} to tune our model on CIFAR-10 dataset. We use SGD with $\eta=0.03$ and $N_v=2$ for $392$ steps, $|B|=256$. The training curves we reported are selected from the best combination from the following hyperparameters $\mathrm{lr}=\{0.005, 0.01\}$, $\mathrm{weight\; decay}=\{10^{-5}, 10^{-4}\}$. We used RandAugment\citep{cubuk2020RandAug}, horizontal flip, Mixup with $\alpha=0.8$ \citep{zhang2018mixup} and Repeated-augmentation \citep{hoffer2020aug}. All of our results are obtained using a single NVIDIA RTX 3090 GPU.

\Cref{fig:vgg}: We use \cref{alg:j_train} to tune our model on CIFAR-10 dataset for $392$ steps with $\eta=0.01$  $|B|=128$ and $N_v=3$. The training curves we reported are selected from the best combination from the following hyperparameters $\mathrm{lr}=\{0.001, 0.002, 0.005, 0.01, 0.02\}$, $\mathrm{weight\; decay}=\{0.0005, 0.001, 0.002, 0.005 \}$. We used RandAugment\citep{cubuk2020RandAug}, horizontal flip and Mixup with $\alpha=0.8$ \citep{zhang2018mixup} and Repeated-augmentation \citep{hoffer2020aug}. We froze auxiliary parameters instead of scale the weights. All of our results are obtained using a single NVIDIA RTX 3090 GPU.

\Cref{figapp:relu_jac}: Exactly the same as \Cref{fig:relu_jac}, except we used JSL.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Theoretical Details}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Factorization of APJN}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We the factorization property using MLP networks in infinite width limit. This proof works for any iid $\theta^l$ where $|\theta^l|$ has some $2+\delta$ moments.

We start from the definition of the partial Jacobian, set $a^l_{\theta}=1$ for simplicity.
\begin{align}
    \nonumber
    \mathcal{J}^{l,l+2} &\equiv \frac{1}{N_{l+2}} \mathbb E_{\theta} \left[ \sum_{i=1}^{N_{l+2}}\sum_{j=1}^{N_{l}} \frac{\partial h^{l+2}_i}{\partial h^{l}_j} \frac{\partial h^{l+2}_i}{\partial h^{l}_j} \right ] \\
    \nonumber
    &= \frac{1}{N_{l+2}} \mathbb E_{\theta} \left[ \sum_{i=1}^{N_{l+2}}\sum_{j=1}^{N_l} \sum_{k,m=1}^{N_{l+1}} 
    \left(W^{l+2}_{ik} \phi'(h^{l+1}_k) \right)
    \left(W^{l+2}_{im} \phi'(h^{l+1}_m) \right)
    \left(\frac{\partial h^{l+1}_k}{\partial h^{l+1}_j} \frac{\partial h^{l+1}_m}{\partial h^{l}_j}\right)
    \right ] \\
    \nonumber
    &= \frac{\sigma_w^2}{N_{l+2} N_{l+1}} \sum_{i=1}^{N_{l+2}}\sum_{j=1}^{N_{l}} \sum_{k=1}^{N_{l+1}} \mathbb E_{\theta} \left[  \phi'(h^{l+1}_k) \phi'(h^{l+1}_k)
    \frac{\partial h^{l+1}_k}{\partial h^{l}_j}
    \frac{\partial h^{l+1}_k}{\partial h^{l}_j} \right ] \\
    \nonumber
    &= \frac{\sigma_w^2}{N_{l+2} N_{l+1}} \sum_{i=1}^{N_{l+2}}\sum_{j=1}^{N_{l}} \sum_{k=1}^{N_{l+1}} \mathbb E_{W^{l+1}, b^{l+1}} \left[ \phi'(h^{l+1}_k) \phi'(h^{l+1}_k)
    W^{l+1}_{kj}  W^{l+1}_{kj} \right] \mathbb E_{\theta} \left[\phi'(h^l_k) \phi'(h^l_k) \right ] \\
    &= \mathcal J^{l,l+1} \mathcal J^{l+1, l+2} + O\left(\frac{\chi^l_{\Delta}}{N_l} \right) \,,
\end{align}
where the $1/N_l$ correction is zero in the infinite width limit. We used the fact that in infinite width limit $h^{l+1}_k$ is independent of $h^l_k$, and calculated the first expectation value of the fourth line using integration by parts. Recall that for a single input (omit x)
\begin{align}
    \chi^{l}_{\Delta} \equiv (a_W^{l+1} \sigma_w)^2 \mathbb E_{\theta} \left[\phi''(h^{l}_i) \phi''(h^{l}_i) + \phi'(h^{l}_i) \phi'''(h^{l}_i) \right] \,.
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Exploding and Vanishing Gradients}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We show details for deriving \eqref{eq:tauto_aw} for MLP networks, assuming $l'>l$:
\begin{align}
    \frac{\partial \log \mathcal J^{l',l'+1}}{\partial a_W^{l+1}} =& \frac{1}{\mathcal J^{l',l'+1}}\frac{\partial \mathbb E_{h^{l'}_i \sim \mathcal N(0, \mathcal K^{l'}(x,x))} \left[(a_W^{l'+1} \sigma_w)^2 \phi'(h^{l'}_i) \phi'(h^{l'}_i) \right]}{\partial a_W^{l+1}} \nonumber \\
    =& \frac{1}{\mathcal J^{l',l'+1}}\frac{\partial}{\partial K^{l'}(x,x)} \left(\frac{{(a_W^{l'+1} \sigma_w)^2}}{\sqrt{2\pi \mathcal K^{l'}(x,x)}} \int \phi'(h^{l'}_i) \phi'(h^{l'}_i) e^{-\frac{h^{l'}_i h^{l'}_i}{2\mathcal K^{l'}(x,x)}} dh^{l'}_i \right) \frac{\partial K^l(x,x')}{\partial a_W^{l+1}}\nonumber \\
    =& \frac{2}{\mathcal J^{l',l'+1}} \chi^{l'}_{\Delta} \frac{\partial \mathcal K^{l'}(x, x)}{\partial \mathcal K^{l'-1}(x,x)} \cdots \frac{\partial \mathcal K^{l+1}(x,x)}{\partial a_W^{l+1}} \nonumber \\
    =& \frac{4}{a_W^{l+1} \mathcal J^{l',l'+1}} \chi^{l'}_{\Delta} \chi^{l'-1}_{\mathcal K} \cdots \chi^{l+1}_{\mathcal K} \mathcal K^{l+1}(x,x) \,,
\end{align}
where we calculated the derivative respect to $\mathcal K^{l'}(x,x)$, then used integration by parts to get the third line. The derivation for \eqref{eq:tauto_ab} is similar.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{ReLU Details}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Learning rate $\eta$} The learning rate bound \eqref{eq:eta_t} is obtained by requiring $|\sqrt{\mathcal J^{l,l+1}(t)} -1 |$ to decrease monotonically with time $t$.

\paragraph{\texorpdfstring{Derivation for $\chi_{\Delta}^l=0$}{}} This is straightforward to show by direct calculation in the infinite width limit. We set $a_W^l=1$ and ignore neuron index $i$ for simplicity. 
\begin{align}
    \chi^{l'}_{\Delta} =& \sigma_w^2 \mathbb E_{h^l \sim \mathcal N(0, \mathcal K^l(x,x))} \left[\phi''(h^{l}) \phi''(h^{l}) + \phi'(h^{l}) \phi'''(h^{l'}) \right] \nonumber \\
    &= \sigma_w^2 \mathbb E_{h^l \sim \mathcal N(0, \mathcal K^l(x,x))} \left [ \frac{d}{dh^{l}} \left( \phi'(h^l) \phi''(h^l)  \right) \right ] \nonumber \\
    &= \sigma_w^2 \mathbb E_{h^l \sim \mathcal N(0, \mathcal K^l(x,x))} \left [ \frac{d}{dh^{l}} \left( \Theta(h^l) \delta(h^l)  \right) \right ] \nonumber \\
    &= \sigma_w^2 \mathbb E_{h^l \sim \mathcal N(0, \mathcal K^l(x,x))} \left [ \frac{h^l}{\mathcal K^l(x,x)} \left( \Theta(h^l) \delta(h^l)  \right) \right ] \nonumber \\
    &= 0 \,,
\end{align}
where $\Theta(h^l)$ is Heaviside step function and $\delta(h^l)$ is Dirac delta function. To get the last line we used $h^l \delta(h^l)=0$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\texorpdfstring{\Cref{conj:bn}}{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here we offer an non-rigorous explanation for the conjecture in the infinite $|B|$ and the infinite width limit. We use a MLP model with $a_{\theta}^l=1$ as an example.

We consider
\begin{align}
    h^{l+1}_{x; i} = \sum_{j=1}^N W^{l+1}_{ij} \phi(\tilde h^l_{x; j}) + b^{l+1}_j + \mu h^l_{x; j}\,,
\end{align}
where 
\begin{align}\label{eq:BN}
    \tilde h^l_{x; i} =& \frac{h^l_{x; i} - \frac{1}{|B|}\sum_{x' \in B} h^l_{x'; i} }{\sqrt{\frac{1}{|B|} \sum_{x' \in B} \left( h^l_{x'; i} \right)^2 - \left(\frac{1}{|B|} \sum_{x' \in B} h^l_{x'; i}\right)^2  }} \nonumber \\
    =& \frac{\sqrt{|B|} \sum_{x' \in B} P_{x x'} h^l_{x'; i}}{\sqrt{ \sum_{x \in B} \left(\sum_{x' \in B} P_{x x'} h^l_{x'; i}\right)^2 }} \,,
\end{align}
where $P_{xx'} \equiv \delta_{xx'} - 1/ |B|$. It is a projector in the sense that $\sum_{x' \in B} P_{xx'} P_{x'x''} = P_{xx''}$.

Derivative of the normalized preactivation:
\begin{align}
    \frac{\partial \tilde h^l_{x; i}}{\partial h^l_{x';j}} = \sqrt{|B|} \left(\frac{P_{xx'}}{\sqrt{\sum_{x \in B} \left(\sum_{x'' \in B} P_{x,x''} h^l_{x'';i}\right)^2}} - \frac{\sum_{x'' \in B} P_{xx''} h^l_{x''; i} \sum_{x'' \in B} P_{x'x''} h^l_{x''; i}}{\left( \sqrt{\sum_{x\in B} \left(\sum_{x'' \in B} P_{x,x''} h^l_{x'';i}\right)^2 } \right)^3} \right)\delta_{ij} \,.
\end{align}

Then the one layer APJN:
\begin{align}\label{eqapp:bn_apjn}
    \mathcal J^{l, l+1} =& \frac{\sigma_w^2}{N_l} \sum_{x,x' \in B} \sum_{j=1}^{N_l} \mathbb E_{\theta} \left[\left(\phi'(\tilde h^l_{x; j}) \right)^2 \left(\frac{P_{xx'}}{\sqrt{\sum_{x \in B} \left(\sum_{x'' \in B} P_{x,x''} h^l_{x''; j}\right)^2}} \right. \right. \nonumber \\
    &\left. \left.- \frac{\sum_{x'' \in B} P_{xx''} h^l_{x''; j} \sum_{x'' \in B} P_{x'x''} h^l_{x''; j}}{\left( \sqrt{\sum_{x \in B} \left(\sum_{x'' \in B} P_{x,x''} h^l_{x''; j}\right)^2 } \right)^3} \right)^2 \right] + \mu^2 \,.
\end{align}

In the infinite $|B|$ limit, only one term can contribute:
\begin{align}
    \mathcal J^{l, l+1} =& \frac{\sigma_w^2}{N_l} \mathbb E_{\theta} \left[\sum_{x,x' \in B} \sum_{j=1}^{N_l} \left(\phi'(\tilde h^l_{x; j}) \right)^2 \frac{P_{xx'} P_{xx'}}{\sum_{x=1}^B \left(\sum_{x'' \in B} P_{x x''} h^l_{x''; j}\right)^2}\right]  + \mu^2 + O\left(\frac{1}{|B|}\right) \nonumber \\
    =& \frac{\sigma_w^2}{N_l} \mathbb E_{\theta} \left[ \sum_{j=1}^{N_l} \sum_{x \in B} \left(\phi'(\tilde h^l_{x; j}) \right)^2 \frac{P_{xx}}{\sum_{x \in B} \left(\sum_{x'' \in B} P_{x x''} h^l_{x''; j}\right)^2} \right] + \mu^2 + O\left(\frac{1}{|B|}\right) \nonumber \\
    =& \frac{\sigma_w^2}{N_l} \mathbb E_{\theta} \left[\sum_{j=1}^{N_l} \left( \left[\frac{1}{|B|} \sum_{x \in B} \left(\phi'(\tilde h^l_{x; j}) \right)^2 \right] \frac{|B|-1}{\sum_{x \in B} \left(\sum_{x'' \in B} P_{x x''} h^l_{x''; j}\right)^2} \right) \right] + \mu^2 + O\left(\frac{1}{|B|}\right) \nonumber \\
    \xrightarrow{B \rightarrow \infty} & \frac{\sigma_w^2}{N_l} \sum_{j=1}^{N_l} \mathbb E_{\tilde h^l_{x;j} \sim \mathcal N(0,  \delta_{xx'} )} \left[\phi'(\tilde h^l_{x;j}) \phi'(\tilde h^l_{x;j}) \right] \frac{1}{\mathcal K^l_{xx} - \mathcal K^l_{xx'}} + \mu^2 \,,
\end{align}
where $x'$ is a dummy index, just to label the off-diagonal term. We used \cref{conjecture:proj} and \cref{conjecture:tilde_h} to get the result.

\begin{conjecture}[Projected Norm]\label{conjecture:proj}
    In the infinite width limit. For a large depth $l$, $\frac{1}{|B|} \sum_{\hat{x} \in B} \left(\sum_{x' \in B} P_{\hat{x}x'} h^l_{x';j}\right)^2$ converges to a deterministic value $\frac{|B|-1}{|B|} \left(\mathcal K^l_{x'x'} - \mathcal K^l_{x' x''} \right)$ as batch size $|B| \rightarrow \infty$.
\end{conjecture}
\begin{proof}[Non-regirous "proof"]
    In the infinite width limit $h^l_{x; j}$ is sampled from a Gaussian distribution $\mathcal N(0, \mathcal K^l_{xx'})$, where the value $\mathcal K_{xx'}$ only depends on if $x$ is the same as $x'$ or not. 

    We first simplify the formula:
    \begin{align}\label{eq:proj}
        &\frac{1}{|B|} \sum_{\hat{x} \in B} \left(\sum_{x' \in B} P_{\hat{x}x'} h^l_{x';j}\right)^2  \nonumber \\
        =& \frac{1}{|B|} \sum_{x', x'' \in B} P_{x' x''} h^l_{x'; j} h^l_{x''; j} \nonumber \\
        =& \frac{1}{|B|} \left(\sum_{x' \in B} (h^l_{x'; j})^2 - \frac{1}{|B|} \sum_{x', x'' \in B} h^l_{x';j} h^l_{x'';j} \right) \nonumber \\
        =& \frac{1}{|B|} \left(\frac{|B|-1}{|B|} \sum_{x' \in B} (h^l_{x'; j})^2 - \frac{1}{|B|} \sum_{x' \neq x''}^B h^l_{x';j} h^l_{x'';j} \right) \,.
    \end{align}    
    The average over $x'$ and $x''$ in infinite $|B|$ limit can be replaced by integration over their distribution (this is the non-rigorous step, complete rigorous proof see \citet{yang2018mean}):
    \begin{align}
        &\frac{1}{|B|} \sum_{\hat{x} \in B} \left(\sum_{x' \in B} P_{\hat{x}x'} h^l_{x';j}\right)^2 \nonumber \\
        \xrightarrow{|B| \rightarrow \infty} & \frac{|B|-1}{|B|}  \left(\mathbb E_{h^l_{x';j} \sim \mathcal N(0, \mathcal K^l_{xx'}) } \left[(h^l_{x'; j})^2 \right] - \mathbb E_{h^l_{x';j} \sim \mathcal N(0, \mathcal K^l_{x'x''}) } \left[h^l_{x';j} h^l_{x'';j} \right] \right) \nonumber \\
        = & \frac{|B|-1}{|B|} \left(\mathcal K^l_{x'x'} - \mathcal K^l_{x' x''} \right) \,,
    \end{align}
\end{proof}

Next, we need to show how to calculate $\mathcal K^{l}_{xx'}$. Before that we first try to simplify find the distribution of $\tilde h^l_{x; i}$ in the infinite $|B|$ limit. 

\begin{conjecture}[$\tilde h^l_{x;i}$ distribution]\label{conjecture:tilde_h}
    In the infinite $|B|$ limit and the infinite width limit, assume for large depth $\mathcal K^l_{xx}$ reaches a fixed point. Then $\tilde h^l_{x;i}$ can be seen as sampled from a Gaussian distribution with the covariance matrix
    \begin{align}
        \lim_{|B| \rightarrow \infty} \mathbb E_{\theta} \left[\tilde h^l_{x;i} \tilde h^l_{y;j}\right] = & \mathbb E_{\theta} \left[ \frac{\sum_{x', x'' \in B} P_{x x'} P_{y x''} h^l_{x';i} h^l_{x'';j}}{\frac{|B|-1}{|B|} \left(\mathcal K^l_{xx} - \mathcal K^l_{x \hat{x}}\right)} \right] \nonumber \\
        =& \frac{\sum_{x', x'' \in B} P_{xx'} P_{yx''} \mathcal K^l_{xx'}}{\frac{|B|-1}{|B|} \left(\mathcal K^l_{xx} - \mathcal K^l_{x \hat{x}}\right)} \delta_{ij} \nonumber \\
        =& \frac{\mathcal K^l_{xy} - \frac{1}{|B|} \mathcal K^l_{\hat{x}\hat{x}} - \frac{|B|-1}{|B|} \mathcal K^l_{x\hat{x}}}{\frac{|B|-1}{|B|} \left(\mathcal K^l_{xx} - \mathcal K^l_{x \hat{x}}\right)} \delta_{ij} \nonumber \\
        =&\delta_{xy} \delta_{ij} \,\,
    \end{align}
    where we used \cref{conjecture:proj} in the first line.
\end{conjecture}

For ReLU:
\begin{align}
    \mathcal K^{l+1}_{xx'} = \begin{cases}
        \frac{\sigma_w^2}{2} + \sigma_b^2 + \mu^2 \mathcal K^l_{xx} & \text{if $x=x'$} \\
        \frac{\sigma_w^2}{2\pi} + \sigma_b^2 + \mu^2 \mathcal K^l_{xx'} & \text{if $x \neq x'$} \,.
    \end{cases}
\end{align}
Then for $\mu=0$ APJN is independent of $\sigma_w^2$ and $\sigma_b^2$ in infinite $|B|$ limit:
\begin{align}
    \mathcal J^{l, l+1} = \frac{\pi}{\pi - 1} \,,
\end{align}
and for $\mu=1$:
\begin{align}
    \mathcal J^{l, l+1} = 1 + O \left(\frac{1}{l} \right) \,.
\end{align}
It is also intuitively clear by realizing the denominator of \eqref{eqapp:bn_apjn} is growing with $l$ when $\mu=1$. Thus the finite $|B|$ corrections are further suppressed. We checked our results in \Cref{fig:bn_relu}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{JSL and JKL}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{JSL}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Since we already discussed our results for JL, we show details for JSL in this section. Derivation for JL is almost identical.

Using JSL, The SGD update of $a^l_{\theta}$ at time t is
\begin{align}\label{eqapp:a_update_jsl}
    a_{\theta}^{l+1}(t+1) - a_{\theta}^{l+1}(t) = - \eta \sum_{l' \geq l}^L  \frac{\partial \mathcal J^{l', l'+1}(t)}{\partial a_{\theta}^{l+1}(t)} \left(\mathcal J^{l', l'+1}(t) - 1 \right) \,.
\end{align}
We focus on ReLU networks to demonstrate the difference between JL and JSL. 

For ReLU networks, we can rewrite \eqref{eqapp:a_update_jsl} as
\begin{align}\label{eqapp:j_update_jsl}
    \sqrt{\mathcal J^{l,l+1}(t+1)} - \sqrt{\mathcal J^{l,l+1}(t)} = -\eta \sigma_w^2 \sqrt{\mathcal J^{l,l+1}(t)} \left(\mathcal J^{l,l+1}(t) - 1\right) \,.
\end{align}

\paragraph{Learning Rate $\eta$} The learning rate limit $\eta_t$ is obtained by requiring $|\sqrt{\mathcal J^{l,l+1}(t)} - 1|$ monotonically decrease with time $t$, for any $l$, then we have
\begin{align}\label{eqapp:eta_t_jsl}
    \eta_t < \min_{1 \leq l \leq L} \left\{\frac{2}{\sigma_w^2 \sqrt{\mathcal J^{l,l+1}(t)} \left(1 + \sqrt{\mathcal J^{l, l+1}(t)}\right)} \right \} \,.
\end{align}

Or by solving \eqref{eqapp:j_update_jsl} with $J^{l,l+1}(1)=1$:
\begin{align}
    \eta_{\mathrm{1-step}} = \frac{1}{\sigma_w^2 \sqrt{\mathcal J^{l,l+1}(0)} \left(1 + \sqrt{\mathcal J^{l, l+1}(0)}\right)}  \,.
\end{align}

For the dynamics of the optimization while using a single learning rate $\eta$. We again estimate the allowed maximum learning rate $\eta_0$ at $t=0$ using $\mathcal J^{l, l+1}(0) = (a_W^{l+1} \sigma_w)^2 / 2$:
\begin{align}
    \eta_0 = \frac{4}{\sigma_w^3 a_W^l \left(\sqrt{2} + a_W^l \sigma_w \right)} \,.
\end{align}

Compared to \eqref{eq:eta_0_jl}, which scales as $1/\log \sigma_w$ for large $\sigma_w$, $\eta_0$ for JSL scales as $\sigma_w^{-4}$ for large $\sigma_w$. This makes the JSL a way worse choice than JLE when $\mathcal J^{l,l+1} \gg 1$.

In \Cref{figapp:relu_jac}, we checked our results with \cref{alg:j_train} using JSL. All other details are the same as \Cref{fig:relu_jac}. The gap between $\eta_0$ and trainable regions can again be explained similarly by analyzing \eqref{eqapp:eta_t_jsl}. Assuming at time $t$: $|\mathcal J^{l,l+1}(t) - 1| < |\mathcal J^{l,l+1}(0) - 1|$ holds. For $\mathcal J^{l,l+1} < 1$ if we use a learning rate $\eta$ that satisfies $\eta_0 > \eta > \eta_t$, there is still a chance that \Cref{alg:j_train} diverges for some $t>0$. For $\mathcal J^{l,l+1} > 1$ if $\eta_0 < \eta < \eta_t$ holds, \Cref{alg:j_train} may say still have a chance to converge for some $t>0$. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{Figures/relu_jacbackprop_jsl.pdf}
    \caption{$\mathcal J^{l, l+1}(t)$ plot for $L=10$, $N_l=500$ ReLU MLP networks, initialized with $a_W^l=1$. From left to right: 1) $\mathcal{J}^{l, l+1}(t=1)$ values are obtained by tuning with \Cref{alg:j_train} using $\eta_{\mathrm{1-step}}$ with JSL; 2) we scan in $\eta$-$\sigma_w$ plane using $\sigma_b=0$ networks, tune $\mathcal J^{l, l+1}(t)$ using \Cref{alg:j_train} with JSL for $980$ steps. Only $0.8< \mathcal J^{l,l+1} <1.25$ points are plotted;  All networks are trained with normalized CIFAR-10 dataset, $|B|=256$.}
    \label{figapp:relu_jac}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{JKL}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We mentioned the following loss function in the main text.
\begin{align}\label{eqapp:jkle}
    \mathcal L_{\mathcal J \mathcal K\log} = \frac{1}{2} \sum_{l=1}^{L} \left[\log(\mathcal J^{l, l+1})\right]^2 + \frac{\lambda}{2} \sum_{l=1}^{L} \left[\log\left (\frac{\mathcal K^{l+1}(x, x)}{\mathcal K^l(x,x)} \right)\right]^2 \,.
\end{align}
There are other possible choices for controlling the forward pass, we will discuss this one briefly.

First we calculate the derivative from kernel terms. We omit $x$ and $t$ dependency and introduce $r^{l+1, l} = \mathcal K^{l+1} / \mathcal K^l$ for clarity:
\begin{align}
    &\frac{\partial}{\partial a_W^{l+1}}\left( \frac{\lambda}{2} \sum_{l'\geq l}^{L} \left[\log{r^{l'+1,l'}}\right]^2 \right) \nonumber \\
    =& \frac{2\lambda}{a_W^{l+1}} \log r^{l+1,l} + \frac{\partial}{\partial a_W^{l+1}}\left( \frac{\lambda}{2} \sum_{l' > l}^{L} \left[\log{r^{l'+1,l'}}\right]^2 \right) \,,
\end{align}
which has a similar structure as APJN terms. Next we pick a term with $l' > l$ in the parentheses:
\begin{align}
    &\frac{\partial}{\partial a_W^{l+1}}\left( \frac{\lambda}{2} \left[\log{r^{l'+1,l'}}\right]^2 \right) \nonumber \\
    =& \frac{\lambda}{\mathcal K^{l'+1} \mathcal K^{l'}} \left(\mathcal K^{l'} \frac{\partial \mathcal K^{l'+1}}{\partial a_W^{l+1}} - \mathcal K^{l'+1} \frac{\partial \mathcal K^{l'}}{\partial a_W^{l+1}}\right)\log{r^{l'+1,l'}} \,,
\end{align}
which is independent of depth for $\sigma_b=0$, and is always finite for $\sigma_b$.

We find that update from the forward pass term for $a_b^{l+1}$ is subtle. For $\sigma_b=0$, similar to the discussion of APJN terms, the update of $a_b^{l+1}$ is zero. For $\sigma_b > 0$, there are two possibilities:
\begin{itemize}
    \item Unbounded activation functions, when $\chi_{\mathcal K}^l > 1$: $\mathcal K^l \rightarrow \infty$ as $l\rightarrow \infty$, thus updates of $a_b^{l+1}$ from the forward pass term vanishes.
    \item Bounded activation functions or unbounded activation functions with $\chi_{\mathcal K}^l < 1$: $\mathcal K^l \rightarrow \mathcal K^{\star}$, thus the contribution from the forward pass term is always $O(1)$.
\end{itemize}
Summarizing the discussion above, we do not have exploding and vanishing gradients problem originated from the term we introduced to tune the forward pass. The forward pass term simply speeds the update of $a_W^{l+1}$ and $a_b^{l+1}$ in most cases.

\paragraph{ReLU} Again we use a ReLU MLP network as an example. 

For $\sigma_b=0$, $\mathcal L_{\mathcal J \mathcal K \log}$ is equivalent to $(1+\lambda)\mathcal L_{\log}$ due to the scale invariance property of the ReLU activation function, which can be checked by using $\mathcal K^{l+1}(x,x) = \sigma_w^2 \mathcal K^l(x,x) / 2$.

For finite $\sigma_b$, we use $\mathcal K^{l,l+1}(x,x) = \mathcal J^{l,l+1} \mathcal K^l(x,x) + \sigma_b^2$:
\begin{align}\label{eqapp:relu_jkl}
    \mathcal L_{\mathcal J \mathcal K \log} = \frac{1}{2} \sum_{l=1}^{L} \left[\log(\mathcal J^{l, l+1})\right]^2 + \frac{\lambda}{2} \sum_{l=1}^{L} \left[\log\left (\mathcal J^{l,l+1} + \frac{\sigma_b^2}{\mathcal K^l(x,x)} \right)\right]^2 \,.
\end{align}

In ordered phase $\mathcal J^{l,l+1} = (a_W^{l+1}(t) \sigma_w)^2 / 2 < 1$, one can prove that $\mathcal K^l(x,x) \rightarrow \sigma_b^2 /(1 - (a_W^{l+1}(t)\sigma_w)^2/2)$ as $l \rightarrow \infty$, thus \eqref{eqapp:relu_jkl} is equivalent to JL at large depth.

In chaotic phase $\mathcal J^{l,l+1} = (a_W^{l+1}(t) \sigma_w)^2 / 2 > 1$ and $\mathcal K^l(x,x) \rightarrow \infty$. \eqref{eqapp:relu_jkl} is equivalent to JL with an extra overall factor $1+\lambda$ at large depth.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ResMLP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%
\subsection{Network Recursion Relation}
%%%%%%%%%%%%%%%%%%

\paragraph{Input} The input image is chopped into an $N \times N$ grid of patches of size $P\times P$ pixels (often $16 \times 16$). The patches are fed into (the same) Linear layer to form a set of $N^2$ $d$-dimensional embeddings, referred to as channels. The resulting input to the ResMLP blocks : $h^0_{\mu i} \in \mathbb R^{N^2} \otimes \mathbb R^{d}$. Here and in what follows, Greek letters ($\mu,\nu$ etc.) index the patches, while Latin letters ($i,j$ etc.) index the channels. Note that in practice, the above two operations are combined into a Convolutional layer with the filer size coinciding with the patch-resolution ($P \times P \times C$); and the stride equal to $P$ so as to avoid overlap between patches. Here, $C$ is the number of channels in the original image.

\paragraph{ResMLP block} The input embedding $h^0_{\mu i}$ is passed through a series of ($L$) self-similar ResMLP blocks, which output $h^L_{\mu i} \in \mathbb R^{N^2} \otimes \mathbb R^{d}$. In the following, we use the notation $1^{2,3}_{4}$ for the parameters; where 1 denotes the parameter, 2 denotes the block-index, 3 denotes the specific action within the block, and 4 denotes the neural indices. A ResMLP block consists of the following operations.
\begin{align}\label{appeq:resmlp_rec_full}
    &\texttt{AffineNorm1:} & a^{l+1}_{\mu i} &= \left( \alpha^{{l+1},a}_i h^{l+1}_{\nu i} + \beta^{{l+1},a}_i \right) \,, & &\left( \mathbb R^{N^2} \otimes \mathbb R^d \right) \\
    &\texttt{linear1:} & b^{l+1}_{\mu i} &= \sum^{N^2}_{\nu=1} W^{{l+1},b}_{\mu\nu} a^{l+1}_{\nu i} + B^{{l+1},b}_{\mu} \,, & &\left( \mathbb R^{N^2} \otimes \mathbb R^d \right) \\
    &\texttt{residual1:} & c^{l+1}_{\mu i} &= \mathcal E^{{l+1},c}_i b^{l+1}_{\mu i} + \mu_1 a^{l+1}_{\mu i} \,, & &\left( \mathbb R^{N^2} \otimes \mathbb R^d \right) \\
    & \texttt{AffineNorm2:} & d^{l+1}_{\mu i} &= \left( \alpha^{{l+1},d}_i c^{l+1}_{\mu i} + \beta^{{l+1},d}_i \right) \,, &&\left( \mathbb R^{N^2} \otimes \mathbb R^d \right) \\
    &\texttt{linear2:} & e^{l+1}_{\mu i} &= \sum^d_{j=1} W^{{l+1},e}_{ij} d^{l+1}_{\mu j} + B^{{l+1},e}_{i} \,, & &\left( \mathbb R^{N^2} \otimes \mathbb R^{4d} \right) \\
    &\texttt{activation:} & f^{l+1}_{\mu i} &= \phi\left(e^{l+1}_{\mu j} \right) \,, & &\left( \mathbb R^{N^2} \otimes \mathbb R^{4d} \right) \\
    &\texttt{linear3:} & g^{l+1}_{\mu i} &= \sum^{4d}_{j=1} W^{{l+1},g}_{ij} f^{l+1}_{\mu j} + B^{{l+1},g}_{i}\,, & &\left( \mathbb R^{N^2} \otimes \mathbb R^d \right) \\
    &\texttt{residual2:} & h^{l+1}_{\mu i} &= \mathcal E^{{l+1},h}_i g^{l+1}_{\mu i} + \mu_2 c^{l+1}_{\mu i} \,, & &\left( \mathbb R^{N^2} \otimes \mathbb R^d \right)
\end{align}
where the brackets on the right contain the dimensions of the output of the layers.

We consider linear layers with weights and biases initialized with standard fan\_in. \texttt{linear1} acts on the patches, with parameters initialized as $W^{l+1,a}_{\mu\nu} \sim \mathcal N(0, \sigma_w^2/N)\,; B^{l+1,a}_{\mu} \sim \mathcal N(0, \sigma_b^2)$. \texttt{linear2} acts on the channels, with parameter initialized as $W^{l+1,e}_{ij} \sim \mathcal N(0, \sigma_w^2/\sqrt{d})\,; B^{l+1,e}_i \sim \mathcal N(0, \sigma_b^2)$. \texttt{linear3} also acts on the channels, with parameters initialized as $W^{l+1,g}_{ij} \sim \mathcal N(0, \sigma_w^2/\sqrt{4d})\,; B^{l+1,g}_i \sim \mathcal N(0, \sigma_b^2)$.
GELU is used as the activation function $\phi$.

\texttt{AffineNrom1} and \texttt{AffineNrom2} perform an element-wise multiplication with a trainable vector of weights $\alpha^{l+1,a}_i, \alpha^{l+1,d}_i  \in \mathbb R^d$ and an addition of a trainable bias vector $\beta^{l+1,a}_i, \beta^{l+1,d}_i \in \mathbb R^d$.
Residual branches are scaled by a trainable vector $\mathcal E^{l+1,c}_i, \mathcal E^{l+1,h}_i \in \mathbb R^{d}$ (\texttt{LayerScale}), whereas the skip connections are scaled by scalar strengths $\mu_1$ and $\mu_2$.

\paragraph{Output} The action of blocks is followed by an Average-Pooling layer, to to convert the output to a $d$-dimensional vector. This vector is fed into a linear classifier that gives the output of the network $h^{L+1}_i$.

%%%%%%%%%%%%%%%%%%
\subsection{NNGP Kernel Recursion Relation}
%%%%%%%%%%%%%%%%%%

At initialization, $\alpha^{l+1,a}_i = \alpha^{l+1,d}_i = \mathbf 1_d$ and $\beta^{l+1,a}_i = \beta^{l+1,d}_i = \mathbf 0_d$. Thus, AffineNorm layers perform identity operations at initialization.
\texttt{LayerScale} is initialized as $\mathcal E^{l+1,c}_i = \mathcal E^{l+1,h}_i = \mathcal E \, \mathbf 1_d$, where $\mathcal E$ is chosen to be a small scalar. (For examlpe, $\mathcal E$ is taken to be 0.1 for 12-block ResMLP and $10^{-5}$ for a 24-block ResMLP network.) Additionally, we also take $\mu_1 = \mu_2 = \mu$.

With these simplifications, we can obtain the recursion relation for the diagonal part of the Neural Network Gaussian Process (NNGP) kernel for the ResMLP block-outputs. We note that the the full NNGP kernel $\mathcal K^l_{\mu\nu;ij}$ is a tensor in $\mathbb R^{N^2} \otimes \mathbb R^{N^2} \otimes \mathbb R^{d} \times \mathbb R^{d}$. Here, we focus on its diagonal part $\mathcal K^l_{\mu\mu;ii}$. For clarity, we remove the subscripts ($\mu\mu;ii$). The diagonal part of the NNGP kernel for a block output $h^l_{\mu i}$ is defined as
\begin{align}\label{appeq:remlp_nngpk}
    \mathcal K^l \equiv \mathbb E_\theta \left[ h^l_{\mu i} h^l_{\mu i} \right] \,,
\end{align}
which is independent of its patch and channel indices, $\mu$ and $i$, in the infinite width limit. The recursion relation can be obtained by propagating the NNGP through a block. For clarity, we define NNGP kernel for the intermediate outputs within the blocks. For example, $\mathcal K^{l+1}_a \equiv \mathbb{E}_{\theta} \left[ a^{l+1}_{\mu i} a^{l+1}_{\mu i} \right]$, $\mathcal K^{l+1}_b \equiv \mathbb{E}_{\theta} \left[ b^{l+1}_{\mu i} b^{l+1}_{\mu i} \right]$, etc.
\begin{align}\label{appeq:resmlp_nngpk_rec}
    &\texttt{AffineNorm1:} & \mathcal K^{l+1}_a &= \mathcal K^l \,, \\
    \nonumber
    &\texttt{linear1:} & \mathcal K^{l+1}_b &= \sigma_w^2 \mathcal K^{l+1}_a + \sigma_b^2 \\
    &&&= \sigma_w^2 \mathcal K^l + \sigma_b^2 \,, \\
    \nonumber
    &\texttt{residual1:} & \mathcal K^{l+1}_c &= \mathcal E^2 \mathcal K^{l+1}_b + \mu^2 \mathcal K^l \\
    \nonumber
    &&&= \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \\
    &&&= \left( \mu^2 + \mathcal E^2 \sigma_w^2 \right) \mathcal K^l + \mathcal E^2 \sigma_b^2 \,, \\
    \nonumber
    &\texttt{AffineNorm2:} & \mathcal K^{l+1}_d &= \mathcal K^{l+1}_c \\
    &&&= \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \,, \\
    \nonumber
    &\texttt{linear2:} & \mathcal K^{l+1}_e &= \sigma_w^2 \mathcal K^{l+1}_d + \sigma_b^2 \\
    &&&= \sigma_w^2 \left( \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \right) + \sigma_b^2 \,, \\
    \nonumber
    &\texttt{activation:} & \mathcal K^{l+1}_f &= \frac{\mathcal K^{l+1}_e}{4} + \frac{\mathcal K^{l+1}_e}{2\pi} \arcsin{\left( \frac{\mathcal K^{l+1}_e}{1 + \mathcal K^{l+1}_e} \right)} + \frac{\left( \mathcal K^{l+1}_e \right)^2}{\pi \left( 1 + \mathcal K^{l+1}_e \right) \sqrt{1 + 2\mathcal K^{l+1}_e}} \\
    \nonumber
    &&&\equiv \mathcal G \left[ \mathcal K^{l+1}_e \right] \\
    &&&= \mathcal G \left[ \sigma_w^2 \left( \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \right) + \sigma_b^2 \right] \,, \\
    \nonumber
    &\texttt{linear3:} & \mathcal K^{l+1}_g &= \sigma_w^2 \mathcal K^{l+1}_f + \sigma_b^2 \\
    &&&= \sigma_w^2 \, \mathcal G \left[ \sigma_w^2 \left( \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \right) + \sigma_b^2 \right] + \sigma_b^2 \,, \\
    \nonumber
    &\texttt{residual2:} & \mathcal K^{l+1} &= \mathcal E^2 \mathcal K^{l+1}_g + \mu^2 \mathcal K^{l+1}_c \\
    \nonumber
    &&&= \mathcal \mu^2 \left( \left( \mu^2 + \mathcal E^2 \sigma_w^2 \right) \mathcal K^l + \mathcal E^2 \sigma_b^2 \right) + \\
    \nonumber
    &&& \quad + \mathcal E^2 \, \left\{ \sigma_w^2 \, \mathcal G \left[ \sigma_w^2 \left( \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \right) + \sigma_b^2 \right] + \sigma_b^2 \right\} \\
    \nonumber
    &&&= \left( \mu^4 + \mu^2 \mathcal E^2 \sigma_w^2 \right) \mathcal K^l + (1 + \mu^2) \mathcal E^2 \sigma_b^2 + \\
    &&&\quad + \mathcal E^2 \sigma_w^2 \, \mathcal  G \left[ \sigma_w^2 \left( \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \right) + \sigma_b^2 \right] \,,
\end{align}
where we have defined 
\begin{equation}
    \mathcal G [z] =  \frac{z}{4} + \frac{z}{2\pi} \arcsin{\left( \frac{z}{1 + z} \right)} + \frac{\left( z \right)^2}{\pi \left( 1 + z \right) \sqrt{1 + 2z}} \,.
\end{equation}

Thus, we have a recursion relation, representing $\mathcal K^{l+1}$ in terms of $\mathcal K^l$.

As a side note, if we replace \texttt{GELU} activation function with \texttt{ReLU}, the relation simplifies greatly, offering us intuition. Specifically, $\mathcal G[z]$ gets replaced by $z/2$ in this case. This gives us the following recursion relation for ResMLP with \texttt{ReLU}.
\begin{align}
    \nonumber
    \mathcal K^{l+1} &= \left( \mu^4 + \mu^2 \mathcal E^2 \sigma_w^2 \right) \mathcal K^l + (1 + \mu^2) \mathcal E^2 \sigma_b^2 + \frac{1}{2} \mathcal E^2 \sigma_w^2 \left( \sigma_w^2 \left( \mu^2 \mathcal K^l + \mathcal E^2 \left( \sigma_w^2 \mathcal K^l + \sigma_b^2 \right) \right) + \sigma_b^2 \right) \\
    &= \left( \mu^4 + \mu^2 \mathcal E^2 \sigma_w^2 + \frac{1}{2} \mu^2 \mathcal E^2 \sigma_w^4 + \frac{1}{2} \mathcal E^4 \sigma_w^6 \right) \mathcal K^l + (1 + \mu^2 + \frac{1}{2}\sigma_w^2) \mathcal E^2 \sigma_b^2 + \frac{1}{2} \mathcal E^2 \sigma_w^2 \sigma_b^2
\end{align}

%%%%%%%%%%%%%%%%%%
\subsection{Jacobian Recursion Relation}
%%%%%%%%%%%%%%%%%%
Next, we calculate the APJN for ResMLP, between two consecutive blocks. For clarity, we first derive the expression for the partial derivative of ${l+1}^{th}$ block output $h^{l+1}_{\mu i}$ with respect to $l^{th}$ block output $h^l_{\nu j}$.
\begin{align}\label{appeq:resmlp_derivative}
    \nonumber
    \frac{\partial h^{l+1}_{\mu i}}{\partial h^l_{\nu j}} &= \mathcal E^{l+1,h}_i \frac{\partial g^{l+1}_{\mu i}}{\partial h^l_{\nu j}} + \mu_2 \frac{\partial c^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \\
    \nonumber
    &= \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} W^{l+1,g}_{ik} \frac{\partial f^{l+1}_{\mu k}}{\partial h^l_{\nu j}} + \mu_2 \frac{\partial c^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \\
    \nonumber
    &= \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) \frac{\partial e^{l+1}_{\mu k}}{\partial h^l_{\nu j}} + \mu_2 \frac{\partial c^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \\
    \nonumber
    &= \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} \sum_{m=1}^d W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{km} \frac{\partial d^{l+1}_{\mu m}}{\partial h^l_{\nu j}} + \mu_2 \frac{\partial c^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \\
    \nonumber
    &= \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} \sum_{m=1}^d W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{km} \frac{\partial c^{l+1}_{\mu m}}{\partial h^l_{\nu j}} + \mu_2 \frac{\partial c^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \\
    \nonumber
    &= \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} \sum_{m=1}^d W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{km} \mathcal E^{l+1,c}_m \frac{\partial b^{l+1}_{\mu m}}{\partial h^l_{\nu j}} + \\
    \nonumber 
    &\quad + \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} \sum_{m=1}^d W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{km} \mu_1 \frac{\partial a^{l+1}_{\mu m}}{\partial h^l_{\nu j}} + \mu_2 \mathcal E^{l+1,c}_i \frac{\partial b^{l+1}_{\mu i}}{\partial h^l_{\nu j}} + \mu_2\mu_1 \frac{\partial a^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \\
    \nonumber
    &= \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} \sum_{m=1}^d \sum_{\lambda=1}^{N^2} W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{km} \mathcal E^{l+1,c}_m W^{l+1,b}_{\mu\lambda} \frac{\partial a^{l+1}_{\lambda m}}{\partial h^l_{\nu j}} + \\
    \nonumber
    &\quad + \mathcal E^{l+1,h}_i \sum_{k=1}^{4d} \sum_{m=1}^d W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{km} \mu_1 \delta_{\mu\nu} \delta_{mj} + \\
    \nonumber
    &\quad + \mu_2 \mathcal E^{l+1,c}_i \sum_{\lambda=1}^{N^2} W^{l+1,b}_{\mu\lambda} \frac{\partial a^{l+1}_{\lambda i}}{\partial h^l_{\nu j}} + \mu_2\mu_1 \delta_{\mu\nu} \delta_{ij} \\
    \nonumber
    &= \mathcal E^{l+1,h}_i \mathcal E^{l+1,c}_j \sum_{k=1}^{4d} W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{kj} W^{l+1,b}_{\mu\nu} + \\
    \nonumber
    &\quad + \mu_1 \mathcal E^{l+1,h}_i \delta_{\mu\nu} \sum_{k=1}^{4d} W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{kj} + \mu_2 \mathcal E^{l+1,c}_i \delta_{ij} W^{l+1,b}_{\mu\nu} + \mu_2\mu_1 \delta_{\mu\nu} \delta_{ij} \\
    \nonumber
    &= \mathcal E^2 \sum_{k=1}^{4d} W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{kj} W^{l+1,b}_{\mu\nu} + \mu \mathcal E \delta_{\mu\nu} \sum_{k=1}^{4d} W^{l+1,g}_{ik} \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{kj} + \\
    &\quad + \mu\mathcal E \delta_{ij} W^{l+1,b}_{\mu\nu} + \mu^2 \delta_{\mu\nu} \delta_{ij} \,,
\end{align}
where in the last step, we have used the initial values of the parameters : $\mathcal E^{l+1,c}_i = \mathcal E^{l+1,h}_i = \mathcal E \, \mathbf 1_d$ and $\mu_1 = \mu_2 = \mu$.

Next, we calculate the APJN using \eqref{appeq:resmlp_derivative}. We will perform the calculation in the limit of large $N^2$ and $d$; dropping all the corrections of order $\frac{1}{N^2}$ and $\frac{1}{d}$.

\begin{align}\label{appeq:resmlp_apjn}
    \nonumber
    \mathcal J^{l,l+1} &= \frac{1}{N^2 d} \mathbb E_\theta \left[ \sum_{\mu,\nu}^{N^2} \sum_{i,j}^d \frac{\partial h^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \frac{\partial h^{l+1}_{\mu i}}{\partial h^l_{\nu j}} \right] \\
    \nonumber
    &= \frac{1}{N^2 d} \mathbb E_\theta \left[ \mathcal E^4 \sum_{\mu,\nu}^{N^2} \sum_{i,j}^d \sum_{k,m}^{4d} W^{l+1,g}_{ik} W^{l+1,g}_{im} \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu m}) W^{l+1,e}_{kj} W^{l+1,e}_{mj} W^{l+1,b}_{\mu\nu} W^{l+1,b}_{\mu\nu} + \right. \\
    \nonumber
    &\qquad\qquad\quad \left. + \mu^2\mathcal E^2 \sum_{\mu,\nu}^{N^2} \sum_{i,j}^d \sum_{k,m}^{4d} \delta_{\mu\nu} W^{l+1,g}_{ik} W^{l+1,g}_{im} \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu m}) W^{l+1,e}_{kj} W^{l+1,e}_{mj} + \right. \\
    \nonumber
    &\qquad\qquad\quad \left. + \mu^2\mathcal E^2 \sum_{\mu,\nu}^{N^2} \sum_{i,j}^d \delta_{ij} W^{l+1,b}_{\mu\nu} W^{l+1,b}_{\mu\nu} + \mu^4 \sum_{\mu,\nu}^{N^2} \sum_{i,j}^d \delta_{\mu\nu} \delta_{ij} \right] \\
    \nonumber
    &= \frac{1}{N^2 d} \mathbb E_\theta \left[ \mathcal E^4 \sigma_w^2 \sum_{\mu,\nu}^{N^2} \sum_j^d \sum_k^{4d} \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{kj} W^{l+1,e}_{kj} W^{l+1,b}_{\mu\nu} W^{l+1,b}_{\mu\nu} +  \right. \\
    \nonumber
    &\qquad\qquad\quad \left. + \mu^2\mathcal E^2 \sigma_w^2 \sum_{\mu,\nu}^{N^2} \sum_j^d \sum_k^{4d} \delta_{\mu\nu} \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu k}) W^{l+1,e}_{kj} W^{l+1,e}_{kj} + \right. \\
    \nonumber
    &\qquad\qquad\quad + \left. \mu^2\mathcal E^2 \sigma_w^2 N^2 d + \mu^4 N^2 d \right] \\
    \nonumber
    &= \frac{1}{N^2 d} \mathbb E_\theta \left[ \frac{1}{4} \mathcal E^4 \sigma_w^6 \sum_\mu^{N^2} \sum_k^{4d} \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu k}) + \mu^2\mathcal E^2 \sigma_w^4 \sum_\mu^{N^2} \sum_k^{4d} \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu k}) + \right. \\
    \nonumber
    &\qquad\qquad\quad \left. + (\mathcal E^2 \sigma_w^2 + \mu^2) \mu^2 N^2 d \right] \\
    \nonumber
    &= (\mu^2 + \mathcal E^2 \sigma_w^2) \left( \mu^2 + \mathcal E^2 \sigma_w^4 \mathbb E_\theta \left[ \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu k}) \right] \right) \\
    \nonumber
    &= (\mu^2 + \mathcal E^2 \sigma_w^2) \left( \mu^2 + \mathcal E^2 \sigma_w^4 \, \mathcal H_e [\mathcal K^{l+1}_e] \right) \\
    &= (\mu^2 + \mathcal E^2 \sigma_w^2) \left( \mu^2 + \mathcal E^2 \sigma_w^4 \, \mathcal H [\mathcal K^l] \right) \,,
\end{align}
where we have defined 
\begin{align}
    \nonumber
    \mathcal H_e [\mathcal K^{l+1}_e] &\equiv \mathbb{E}_\theta \left[ \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu k}) \right] \\
    &= \frac{1}{4} + \frac{1}{2\pi} \left( \arcsin{\left( \frac{\mathcal K^{l+1}_e}{1 + \mathcal K^{l+1}_e} \right)} + \frac{\mathcal K^{l+1}_e (3  + 5 \mathcal K^{l+1}_e)}{(1 + \mathcal K^{l+1}_e) (1 + 2\mathcal K^{l+1}_e)^{3/2}} \right) \,.
\end{align}
We also write $\mathcal K^{l+1}_e$ in terms of $\mathcal K^l$ and define
\begin{align}
    \nonumber
    \mathcal H [\mathcal K^l] &= \mathcal H_e [\mathcal K^{l+1}_e] \\
    &= \mathcal H_e \left[ \sigma_w^2 \left( \mu^2 \mathcal K^l + \mathcal E^2 (\sigma_w^2 \mathcal K^l + \sigma_b^2) + \sigma_b^2 \right) \right] \,.
\end{align}

It is clear from \eqref{appeq:resmlp_apjn} that for $\mu=1$, $\mathcal J^{l,l+1} > 1$, rendering the network off criticality. However, $\mathcal J^{l,l+1}$ can be tuned arbitrarily close to criticality by taking $\mathcal E$ to be small at $t=0$. This explains the necessity for \texttt{LayerScale} with small initial value in the ResMLP architecture.

We note that the results in \eqref{appeq:resmlp_apjn} greatly simplify on using \texttt{ReLU} instead of \texttt{GELU} as $\phi$. We mention them here to provide intuition. $\mathcal H_e [\mathcal K^{l+1}_e] = \mathbb{E}_\theta \left[ \phi'(e^{l+1}_{\mu k}) \phi'(e^{l+1}_{\mu k}) \right] = \frac{1}{2}$ in this case. This gives us the simple result
\begin{equation}
    \mathcal J^{l,l+1} = (\mu^2 + \mathcal E^2 \sigma_w^2) \left( \mu^2 + \frac{1}{2}\mathcal E^2 \sigma_w^4 \right) 
\end{equation}
for \texttt{ReLU} activation function.

